When--and how--can a cellular automaton be rewritten as a lattice gas?

Both cellular automata (CA) and lattice-gas automata (LG) provide finite algorithmic presentations for certain classes of infinite dynamical systems studied by symbolic dynamics; it is customary to use the term `cellular automaton' or `lattice gas' for the dynamic system itself as well as for its presentation. The two kinds of presentation share many traits but also display profound differences on issues ranging from decidability to modeling convenience and physical implementability. Following a conjecture by Toffoli and Margolus, it had been proved by Kari (and by Durand--Lose for more than two dimensions) that any invertible CA can be rewritten as an LG (with a possibly much more complex ``unit cell''). But until now it was not known whether this is possible in general for noninvertible CA--which comprise ``almost all'' CA and represent the bulk of examples in theory and applications. Even circumstantial evidence--whether in favor or against--was lacking. Here, for noninvertible CA, (a) we prove that an LG presentation is out of the question for the vanishingly small class of surjective ones. We then turn our attention to all the rest--noninvertible and nonsurjective--which comprise all the typical ones, including Conway's `Game of Life'. For these (b) we prove by explicit construction that all the one-dimensional ones are representable as LG, and (c) we present and motivate the conjecture that this result extends to any number of dimensions. The tradeoff between dissipation rate and structural complexity implied by the above results have compelling implications for the thermodynamics of computation at a microscopic scale.

==> fig/scrap <==
					/GAP 40 \	% gap in ring
					/ring{		% x y % ring at x y
		gs  neiw %[1 45 div]0 sd
		  np RAD 90 GAP add 450 GAP sub arc gr s}\


==> flipbook/split <==
#!/usr/bin/env python

def dopage(n):
  print 'Page %s' % n
  sink = open('../fig/flip%s.eps'%n,'w')
  for i in prolog: sink.write(i)
  while 1:
    i = sors.readline()
    sink.write(i)
    if i[:3]=='eop':
      sink.close(); break


sors = open('2x2book.ps')

prolog = []

while 1:
  i = sors.readline()
  prolog.append(i)
  if i[:11]=='%%EndProlog': break
prolog.append('/eop{}\\\n')

#print ''.join(prolog)

i = sors.readline()
while i:
  if i[:7]=='%%Page:':
#    print i
    n = i.split()[1]
    dopage(n)
  i = sors.readline()


==> py/and2 <==
#!/usr/bin/env python
#-*-fundamental-*- tt 061214 070311 070320 070510
import math

''' Determining the minimum width of an encoder needed to turn the 2-input
AND cellular CA into a LG. Typical commands:
  and -h	# Help with command syntax and usage
  and 4		# Run for n up to 4
  and 		# Run for n up to 12 (default)
  and -d1 4	# Run for n up to 4; display output pattern histogram
  and -d2 4	# Run for n up to 4; display full list of I/O patterns

Choose a linear patch of length n and its preimage patch of length n+1 and
compute one step of the rule over all 2^(n+1) states of the preimage.
Construct the histogram of the states that actually occur in the image, and a
similar histogram where the new state has been augmented by a strip of old
state (in this case just one bit) sufficient for overlap of lattice-gas-like
blocks.
 Tabulate results, giving the variety V (log of the number of distinct
states) and the entropy H (ordinary weighted logarithmic average) of the
histogram, as well as variety W of the augmented histogram.

Two neighbors per site, at -1/2 and +1/2 (we can call this the "HORN"
neighborhood).  The new state of each site is computed by applying the local
map f to the old state of its two neighbors,
	t  :	. . u v w x u z . .	,	where U = f(u,v), etc.
	t+1:     . . U V W X Y . .	
 (In our diagrams we order bits typografically, spatially from LSB on the
left to MSB on the right, as usual in graphics work, and temporally from top
to bottom.)
 Without any loss of generality, It will be convenient to align sites
flush-left, just as when the
		  1   		 1  
Pascal triangle  1 1  is written 11 ,	and write	..uvwxyz.. (U= f(u,v))
  		1 2 1 		 121			..UVWXYZ..	

To make a compressing encoder of output width n that will operate on a block
of length n+1 and, in the transition uv..xy -> UV..X, squeeze a copy of the
first old bit u (needed to sew up the edges of adjacent blocks) into the
lines UV..X that carry the first n bits of the new state---a total of n+1
bits---into only n bits!
 But bit u contributed (as part of the argument) to the result UV..X and in
general will NOT be independent of bits UV. Thus the total amount of variety
to be squeezed into the encoder is not that of UV..X plus that of u
separately, but the joint variety of uUV..X, which may be less. '''

def bin(x, size=8):		
  "Turn integer to binary string with LSB first, for debugging"
  return ''.join(map(lambda y:str((x>>y)&1), range(size)))

def lg2(x): return math.log(x,2)

def make(n):					# n is size of image
  N = 2**(n+1) 					# N is size of table
  M = 2**n					# M is size of histogram
  W = 2**(n+1)					# W is size of extended hist
  Mhist = M*[0]					
  Whist = W*[0]					

  for x in xrange(N):
    y = x&x>>1
    Y = (y<<1)|(x&1)
    Mhist[y] += 1
    Whist[Y] += 1
#    print bin(x,n+1), bin(y,n), bin(Y,n+1)	# For debugging

  hits = 0; sinf = 0; Hits = 0				# 
  for i in Mhist:				# Count hits
    if i:
      hits += 1; sinf += i*lg2(i)
  for i in Whist:				# Count hits
    if i: Hits += 1

  ent = lg2(N)-sinf/N

  print '%2i  %5.2f (%5.3f)   %5.2f  %5.2f/%i   '\
        % (n,ent,ent/n,lg2(hits),lg2(Hits),n+1)

print '                 AND2 in 1 dimension\n'
print ' n    ent   eta      var    xvar/nx\n'  

for k in range(1,17): make(k)


==> py/and_open <==
#!/usr/bin/env python

'''  [with no wraparound]
 Compute one step of 1D CA rule (AND of 2 in this case) over the entire state
set, and report variety and entropy of the resulting state set.
 N is the number of sites. 
 var is a dictionary containing equivalence classes of neighborhood
patterns. Two such patterns are equivalent if they yield the same output
pattern.
 "Variety" counts (in log scale) those equivalence classes, regardless of how
many neighborhood configurations each contains.
 "Entropy" counts (in log scale) those equivalence classes, weighted as per how
many neighborhood configurations each contains.
'''

import sys,getopt
from math import log

def entropy(var):
  S = 0					# Clear entropy
  for i in var:				# Integrate entropy:
    p = float(var[i])/NN		#  weight of item
    S += -p*log(p,2)			#  self-information of item
  return S

def rule(N):	
  'Collect equivalence classes and compute variety and entropy for N sites'
  var = {}				# Clear variety dictionary
  for old in xrange(NN):		# For each neigh pattern (bin integer)
    out = old & XTRA			#  clear out pattern or init to thru bit
    for j in reversed(xrange(N)):	#  run through all sites
      out <<= 1
      out += bool((old&(2**j) and old&(2**(j+1))))
    if DBUG&1: print '%2X %2X' % (old,out)
    if var.has_key(out):
      var[out] += 1
    else: var[out] = 1
  if DBUG&2:
    for i in var: print '%2X:%i ' % (i,var[i]),	# the output pattern range
    print

  V = log(len(var),2)			# total variety
  S = entropy(var)			# total entropy 
  print '%2i  V: %5.2f %5.3f  S: %5.2f %5.3f' % (N,V,V/float(N),S,S/float(N))



#----------------------------------------------------------------
options = '''\
	-h 	help	print this help summary
	-x	xtra	execute with thru bit
	-d n	debug	n is the debug mask, with bits as follows
			  0 print old pattern and output pattern
			  1 print variety dictionary (key and multiplicity)
'''

usage = '  Command: %s [-h] [-x] [-d bin] sites\n%s' % (sys.argv[0],options)

def main():
  opts,args = getopt.getopt(sys.argv[1:],'hxd:')
  global DBUG; DBUG = 0
  global XTRA; XTRA = 0
  for opt in opts:
    if opt[0]=='-h': print usage; sys.exit()# help with usage
    if opt[0]=='-x': XTRA = 1		# Make use of thru bit
    if opt[0]=='-d':
      try: DBUG = opt[1]
      except IndexError:
        print 'No DBUG argument given'; sys.exit()
  try: NMAX = int(args[0])
  except IndexError:
    print 'No argument (max no. of sites) given'; sys.exit()

  for N in range(2,NMAX+1):
    global NN; NN = 2**(N+1)		# no. of sites N + no. of neigh
    rule(N)


main()




==> py/try <==
#!/usr/bin/env python

import sys,getopt

usage = '''\
nonsense'''





def main():
  opts,args = getopt.getopt(sys.argv[1:],'hxd:')

  print opts,args

  for opt in opts:
    if opt[0]=='-h': print usage; sys.exit()# help with usage


main()

==> seminar <==
parisi giorgio*		23481  	giorgio.parisi@roma1.infn.it 	  	F 110
		24311	23401
pietronero luciano*	23488  	pietronero@roma1.infn.it 	  	F 108
petrarca silvano	24376  	Silvano.Petrarca@roma1.infn.it 	  	M 149b
cabibbo nicola		24349  	nicola.cabibbo@roma1.infn.it 	  	M S104
vulpiani angelo*	23840  	angelo.vulpiani@roma1.infn.it 	  	F 208



Antonio Machi'	49913767 	machi@mat.uniroma1.it			mat 137
Tullio Ceccherini 0824305837	tceccher@mat.uniroma1.it


To: giorgio.parisi@roma1.infn.it, tceccher@mat.uniroma1.it,machi@mat.uniroma1.it\
,nicola.cabibbo@roma1.infn.it,pietronero@roma1.infn.it,Silvano.Petrarca@roma1.in\
fn.it,angelo.vulpiani@roma1.infn.it, scoppola@univaq.it
cc: capobian@mat.uniroma1.it, mentrasti@mat.uniroma1.it,Paolo.Lariccia@pg.infn.\
it, stefano.lariccia@uniroma1.it


Subject: prospective seminar on "Cellular automata vs lattice gases:
Numerical integration of symbolic dynamics without using batteries?"
--text follows this line--

Dear Giorgio, Tullio, Antonio, Nicola, Luciano, Silvano, Angelo, Carlo:

Stiamo cercando di organizzare un seminario di un'ora o un po` piu`, magari
anche con pranzo o cena dopo, sui rapporti fra automi cellulari e gas su
reticolo dal punto di vista algebrico e topologico (non quello fenomenologico
di caos e systemi complessi). In questo contesto, ho (insieme con Mentrasti e
Capobianco di Matematica qui) dei risultati interessantissimi dal punto di
vista della modellizzazione della fisica di base---essenzialmente come
integrare numericamente versioni discrete di equazioni differenziali alle
derivate parziali con calcolatori che non richiedono batterie!

In una conferenza del 1981 Richard Feynman disse "Noi fisici facciamo dei
calcoli quantistici complicatissimi per decidere dove si trovera` l'elettrone
all'istante successivo, ma io non sono per niente convinto che l'elettrone si
debba portare dietro un computer per sapere dove andare."  Naturalmente, il
dubbio piu` grave non e` se l'elettrone si porti dietro un computer (che ne
sappiamo noi?) ma DOVE TROVEREBBE LE BATTERIE per farlo funzionare per
miliardi di anni (in un mondo microscopicamente reversibile e percio`
obbediente al secondo principio della termodinamica).  Il nostro risultato e`
che e` possibile calcolarsi la traiettoria di un "symbolic dynamics system",
invertibile o meno, con un computer che non richiede batterie---ma a costo di
usare un computer MOLTO PIU` COMPLICATO di uno equivalente funzionante a
batterie.

Il tema del seminario e` percio` sui rapporti fra struttura e funzione in
sistemi di calcolo distribuiti e uniformi, tenendo conto di aspetti di
disipation, decidability, information theory, and computation complexity su un
sottofondo di topological dynamics.

Stiamo cercando di trovare una finestra (giorno e ora) per Mercoledi o
Venerdi della settimana prossima (July 5 or 7) o al peggio la settimana
successiva. T'interesserebbe partecipare, e nel caso quando preferiresti?
(L'invito e` estendibile a partecipanti qualificati di tua scelta).

Looking forward,

        Tommaso Toffoli                                   Boston University
        Patrizia Mentrasti (host) and Silvio Capobianco   Matematica Roma I




==> smallbib.tex <==
\makeatletter
\renewenvironment{thebibliography}[1]
     {\small \section*{List of references%
%        \@mkboth{\MakeUppercase\bibname}{\MakeUppercase\bibname}%
								}%
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
%            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist\par}
\makeatother
